Fast and exact evaluation of box splines via the PP-form

For the class of non-degenerate box splines, we prove that these box splines are piecewise polynomial. This is not a new result, it is in fact a well known and useful property of box splines. However, our proof is constructive, and the main result of this work is a corollary that follows from this proof, namely one that gives an explicit construction scheme for the polynomial pieces in the interior regions of any non-degenerate box spline.

==> sections/definitions.tex <==
\section{Difference Operator} \label{sec:support}
The difference operator has a simple characterization in the spatial domain which is summarized as followed

\begin{theorem}{1} \label{thm:support_thm}
Let $\bigxi$ be an $s$ by $n$ matrix and define the multi-set $S_{\bigxi}$ recursively by the rules
\begin{equation}
	S_{\left[ \ \right]}:= \left\{(1,\bm{0})\right\} \text{ and } S_{\bigxi} := \left\{ (-c,\bm{\xi} + \bm{p})  : (c,\bm{p}) \in S_{\bigxi \backslash \bm{\xi}} \right\} \cup S_{\bigxi \backslash \bm{\xi} }
\end{equation} 
then the difference operator $\diffxi$ is given by the distribution
\begin{equation}
	\diffxi = \sum_{(c,\bm{p}) \in S_{\bigxi}} c\delta(\cdot - \bm{p})
\end{equation}
where $\delta$ is the Dirac delta distribution.
\end{theorem}

\begin{proof}
We show this inductively on the number of columns of $\bigxi$. 
As a base case, assume $\bigxi$ contains a single non-zero direction vector, $\bm\zeta$, then we have  $\hat{\nabla}_{\bigxi} = 1-\exp(i\bm\zeta\cdot\omega)$ which has the spatial form $\diffxi = \delta - \delta(\cdot - \bm\zeta)$
which is by definition 
\begin{equation}
	\diffxi = \sum_{(c,\bm{p}) \in S_{\bigxi }} c\delta(\cdot - \bm{p}).
\end{equation}

For the general case, pick some $\bigxi$ with $n > 1$ columns, and suppose that for any $\bigxi^\prime$ with $i<n$ columns this results hold. 
Then split $\bigxi$ into an $s$ by $n-1$ matrix $\bigxi^\prime$ and column vector $\bm{\zeta}$, and consider the difference operator $\nabla_{\bigxi^\prime \cup \bm{\zeta}}$.
From the Fourier expression we have 
\begin{equation*}
	\hat{\nabla}_{\bigxi} = \hat{\nabla}_{\bigxi^\prime \cup \bm{\zeta}} = \prod_{\bm{\xi} \in \bigxi^\prime \cup \bm{\zeta}} (1 - \exp\left(-i \bm{\xi} \cdot \bm{\omega})\right) =  \left(1 - \exp(-i \bm{\zeta} \cdot \bm{\omega}) \right) \hat{\nabla}_{\bigxi^\prime}.
\end{equation*}
Which is equivalently stated in the spatial domain as 
\begin{equation}
\diffxi = {\nabla}_{\bigxi^\prime \cup \bm{\zeta}} = \nabla_{\bigxi^\prime} - \nabla_{\bigxi^\prime}(\cdot - \bm{\zeta}).
\end{equation}
The inductive hypothesis then gives
\begin{equation}
{\nabla}_{\bigxi^\prime \cup \bm{\zeta}}= \sum_{(c,\bm{p}) \in S_{\bigxi^\prime}} c \delta(\cdot - \bm{p}) + \sum_{(c,\bm{p}) \in S_{\bigxi^\prime}}  -c\delta(\cdot - (\bm{p} + \bm\zeta) )
\end{equation}
and it follows, by definition of $S_{\bigxi}$, that
\begin{equation}
	\diffxi = {\nabla}_{\bigxi^\prime \cup \bm{\zeta}} = \sum_{(c,\bm{p}) \in S_{\bigxi }} c\delta(\cdot - \bm{p})
\end{equation}
which completes the induction.
\end{proof}

